On Computing Pareto Optimal Paths in Weighted Time-Dependent Networks

A weighted point-availability time-dependent network is a list of temporal edges, where each temporal edge has an appearing time value, a travel time value, and a cost value. In this paper we consider the single source Pareto problem in weighted point-availability time-dependent networks, which consists of computing, for any destination d, all Pareto optimal pairs (t, c), where t and c are the arrival time and the cost of a path from s to d, respectively (a pair (t, c) is Pareto optimal if there is no path with arrival time smaller than t and cost no worse than c or arrival time no greater than t and better cost). We design and analyse a general algorithm for solving this problem, whose time complexity is O(M log P), where M is the number of temporal edges and P is the maximum number of Pareto optimal pairs for each node of the network. This complexity significantly improves the time complexity of the previously known solution. Our algorithm can be used to solve several different minimum cost path problems in weighted point-availability time-dependent networks with a vast variety of cost definitions, and it can be easily modified in order to deal with the single destination Pareto problem. All our results apply to directed networks, but they can be easily adapted to undirected networks with no edges with zero travel time.

==> applicationstable.tex <==
\begin{tabular}{||c||>{\centering}m{3.5cm}|>{\centering\arraybackslash}m{2cm}||}
\hline
\multirow{2}{*}{\textbf{Application}} & \multicolumn{2}{c||}{\textbf{Complexity}}\\
\cline{2-3}
 & \textit{State of the art} & \textit{Algorithm 1}\\
\hline
Profile problem & \makecell{$O(M\log P)$\\ implicit in \cite{Dibbelt2013,Dibbelt2018,Wu2014Path,Wu2016}} & \\
\cline{1-2}
Fewest hops & \makecell{$O(n \cdot m \cdot \log \delta)$\\  \cite{Xuan2003}} & \\
\cline{1-2}
Shortest delay & \makecell{$O(M\log d_{max})$\\  \cite{Wu2014Path,Wu2016}} &  $O(M \log K)$\\
%$d_{max} is the maximum in degree of a node (not topological, counting the total number of connections entering anode)$
\cline{1-2}
Shortest fastest & \makecell{$O(M \log |T|)$\\ \cite{Simard2019}} & \\
%adjust notation
\cline{1-2}
Highest reliability & - &  \\
\cline{1-2}
Min max & - &  \\



\hline
\hline
\end{tabular}

% \begin{tabular}{||c||>{\centering}m{3.5cm}|>{\centering\arraybackslash}m{2cm}||}
% \hline
% \multirow{2}{*}{\textbf{TDN class}} & \multicolumn{2}{c||}{\textbf{Complexity profile problem}}\\
% \cline{2-3}
%  & \textit{Time} & \textit{Profile size}\\
% %\hline
% %TDN & ?? $\Omega(n^{\log n})$  \cite{Foschini2014} & $\Omega(n^{\log n})$\\
% \hline
% Piecewise-linear & \makecell{$O(nPm)$\\ \cite{Orda1990}}
% %$n\times O((P+M)(m+n\log n))$ \cite{Dehne2012}
% & can be $\Omega(n^{\log n})$ \cite{Foschini2014}\\
% \hline
% Constant-delay & \makecell{$O(M(m+n\log n))$\\ \cite{Dehne2012}} & \\
% \cline{1-2}
% Point-availability & \makecell{$O(M\log P)$\\ implicit in \cite{Dibbelt2013,Dibbelt2018,Wu2014Path,Wu2016}} & {$O(M)$}\\
% %\hline
% %Uniform TDN & ?? &\\
% %\hline
% %Integral bounded-delay TDN & $O(M)$ (this paper) &\\
% \cline{1-2}
% Temporal network & \makecell{$O(M)$\\ implicit in \cite{Kossinets2008Structure}} & \\
% \hline
% \hline
% \end{tabular}

==> modelproblem.tex <==
\section{Definitions, network models, and problems}
\label{sec:modelproblem}

A \textit{time-dependent network} (in short, \textit{TDN}) is a graph $G=(V,E)$, where $V$ is the set of $n$ \textit{nodes} and $E\subseteq V\times V$ is the set of $m$ \textit{edges}, along with a total function $\alpha:E\times\thor\rightarrow \mathbb{R}\cup\{\infty\}$ where $\thor\subseteq\mathbb{R}$. For any edge $e=(u,v)\in E$ and for any \textit{time instant} $t\in\thor$, $\alpha(e,t)$ (also denoted as $\alpha_e(t)$) specifies the \textit{arrival time} in $v$ of $e$, if we start from $u$ at time $t$ (if $\alpha(e,t)=\infty$, then it means that the edge $e$ is not available at time $t$). In other words, whenever a path arrives in $u$ at time $t$, if the edge $e$ is then traversed, the path arrives in $v$ at time $\alpha_e(t)$. Note that, in general, the arrival time function of an edge $e$ can be any one-variable function defined over $\thor$ such that, for any $t\in\thor$, $\alpha_e(t)\geq t$ (since we cannot yet travel back in time). For example, in Figure~\ref{fig:timedependentnetwork}, the arrival time function of the edge $e_1$ is the function $-t^2+6t$, which is always above the identity function (represented in dashed in the corresponding plot) if $\thor=[0,5]$.

Given a TDN $N = \langle G=(V,E),\alpha,\gamma,\thor\rangle$, for any edge $e=(u,v)\in E$, we will denote by $\tail e=u$ and $\head e=v$ the tail and the head of the arc $e$, respectively. Given two nodes $u,v\in V$, a \textit{$\sd uv$ walk} $\tpath W$ from $u$ to $v\in V$  is a sequence of edges $\langle e_1,e_2,\ldots,e_k\rangle\subseteq E^k$ such that $u=\tail{e_1}$, $v=\head{e_k}$, and, for each $i$ with $1<i\leq k$, $\tail{e_i}=\head{e_{i-1}}$. A \textit{$\sd uv$ path} $\tpath P$ is a $\sd uv$ walk with pairwise distinct nodes. For any $t\in\thor$, the \textit{arrival time function} of a $\sd uv$ walk $\tpath W=\langle e_1,e_2,\ldots,e_k\rangle$ is defined as
\[
\alpha_{\tpath W}(t)=\alpha_{e_k}(\alpha_{e_{k-1}}(\cdots\alpha_{e_2}(\alpha_{e_1}(t))\cdots)).
\]

As we said in the introduction, in this paper we deal with the \textit{unrestricted waiting} traversal policy, according to which it is possible to wait at a node until some edge with finite arrival time appears and allows us to leave the node. In this case, for each edge $e$ and for all $t\in\thor$ such that $\alpha_e(t)=\infty$, we can consider that the ``real'' arrival time of $e$ at $t$ is equal to $\alpha_e(t')$, where $t'$ is the minimum value greater than $t$ such that $\alpha_e(t')<\infty$ (if such a $t'$ does not exist, then the arrival time does not change). Note that referring to this policy implies that, for any $\sd uv$ walk $\tpath W$, there exists a $\sd uv$ path $\tpath P$ such that, for any $t\in\thor$, $\alpha_{\tpath P}(t)=\alpha_{\tpath W}(t)$. From now on, we can then focus our attention on paths only. If $\allpaths uv$ denotes the set of all $\sd uv$ paths in $G$, the \textit{earliest arrival time} function of $u$ and $v$ is defined as  $\eat uvt=\min_{\tpath P\in\allpaths uv}\alpha_{\tpath P}(t)$.

\problem{The profile problem}{Given a TDN $N = \langle G=(V,E),\alpha,\gamma,\thor\rangle$, and a source node $s\in V$, compute the \textit{profile} of $s$, that is, the function $\pi_s(u,t) = \eat sut$.}

This problem has been very well studied in the literature and its complexity depends on the characteristics of the arrival time function. The above definition of TDN can be, indeed, refined by assuming that, for each edge $e$, the arrival time function $\alpha_e(t)$ is piecewise linear (as for example, in the case of the arrival time functions of the two edges $e_2$ and $e_3$ in Figure~\ref{fig:timedependentnetwork}). More precisely, in a \textit{piecewise linear} TDN $N = \langle G=(V,E),\alpha,\gamma,\thor\rangle$, for each edge $e\in E$, there exists a finite set of disjoint intervals $\mathbb{I}_{e,1}=[l_{e,1},r_{e,1}],\ldots,\mathbb{I}_{e,k_e}=[l_{e,k_e},r_{e,k_e}]$ such that, for each $i$ with $1\leq i\leq k_e$ and for each $t\in\mathbb{I}_{e,i}$, $\alpha_e(t)=a_{e,i}t+b_{e,i}$ for some $a_{e,i},b_{e,i}\in\mathbb{R}$, and, for each $t\not\in\bigcup_{i=1}^{k_e}\mathbb{I}_{e,i}$, $\alpha_e(t)=\infty$.

A special case of piecewise-linear TDN is the \textit{constant-delay} one, which correspond to the case in which, for any edge $e$, all slopes $a_{e,i}$ are equal to $1$. This case is called constant-delay for the following reason. For each edge $e$ and for each time $t$, the \textit{delay} of $e$ at time $t$ is defined as $\alpha_e(t)-t$: hence, the delay corresponds to the travel time of the edge at time $t$. In the case of piecewise linear TDNs, the delay is equal to $a_{e,i}t+b_{e,i}-t=(a_{e,i}-1)t+b_{e,i}$: if all slopes $a_{e,i}$ are equal to $1$, then the delay is constant in each interval (that is, equal to $b_{e,i}$).

The class of constant-delay TDNs can be further restricted by assuming that $\thor$ is a finite set of points. This kind of TDNs is called \textit{point-availability} TDN, and it is the one on which we will focus our attention in the next sections. Note that an equivalent representation of a point-availability TDN $N = \langle G=(V,E),\alpha,\gamma,\thor\rangle$ simply consists in listing all the \textit{temporal edges} of the network, where a temporal edge $e$ is a quadruple $(u_e,v_e,t_e,\delta_e)$, where $(u_e,v_e)\in E$, $t_e\in\thor$, and $\delta_e$ is the delay of $(u_e,v_e)$ at time $t_e$. This is, indeed, the representation we are going to use while describing our algorithms (see also Figure~\ref{fig:pointavailabilitytdn}).

Whenever the delay of each edge $e$ at each time $t$ is the same value $\delta$, we say that the constant-delay TDN is a \textit{uniform} TDN. Typically, the value of $\delta$ is equal either to $1$ (like in the case of the temporal graphs) or to $0$ (like in the case of the finite link streams).

The above hierarchy (see the left part of Figure~\ref{fig:hierarchy}) induces different complexities for the profile problem (see the right part of the figure). The complexity of computing the set of Pareto optimal pairs $(t_{dep},t_{arr})$ ranges from super-polynomial for piecewise linear~\cite{foschini-fixme} to linear for pure availability times. It is $O(M(m+ n\log n))$ for availability intervals~\cite{dehne-fixme} and $O(M\log M)$ for availability times where $n,m,M$ denote the number of nodes, edges and temporal edges respectively. The complexity for availability times can be obtained by analyzing the profile connection scan algorithm~\cite{csa-fixme}. It basically consists in a linear scan of temporal edges (called connections in that context) in appropriate order. The $\log M$ factor comes from the dichotomy search performed for each temporal edge in a sorted vector whose size is upper-bounded by $M$.
\comPC{To be rewritten}

In this paper we extend the definition of a TDN in order to deal with a multiplicity of objectives while computing paths starting from a given source. To this aim, we integrate the definition of a TDN with a \textit{cost function} $\gamma:E\times\thor\rightarrow\cost$ where $\cost$ is the set of possible cost values, a \textit{cost combination function} $\oplus:\cost\times\cost\rightarrow\cost$, and a \textit{cost comparison relation} $\preceq\ \subseteq\ \cost\times\cost$. For any $t\in\thor$, the \textit{cost function} of a $\sd uv$ path $\tpath P=\langle e_1,e_2,\ldots,e_k\rangle$ is recursively defined as follows
\[
\gamma_{\tpath P}(t)=\gamma_{\langle e_1,e_2,\ldots,e_{k-1}\rangle}(t)\oplus\gamma_{e_k}(\alpha_{\langle e_1,e_2,\ldots,e_{k-1}\rangle}(t)),
\]with $\gamma_{\langle e_1\rangle}(t)=\gamma_{e_1}(t)$ (in other words, the costs combine along the path according to the cost combination function). 

The problem we focus on in this paper is then the following one. We want to compute the set of Pareto optimal values of the paths from a given source starting at a given time to all the possible destinations, with respect to two criteria:  arrival time and cost. More precisely, given a time $t_0\in\thor$, a path $\tpath P\in\allpaths sd$ is \emph{Pareto $t_0$-optimal} among all paths in $\allpaths sd$, if there is no path $Q\in\allpaths sd$ such that $\alpha_{\tpath Q}(t_0) < \alpha_{\tpath P}(t_0)$ and $\gamma_{\tpath Q}(t_0) \preceq \gamma_{\tpath P}(t_0)$, or $\alpha_{\tpath Q}(t_0) \leq \alpha_{\tpath P}(t_0)$ and $\gamma_{\tpath Q}(t_0) \prec \gamma_{\tpath P}(t_0)$ (the relation $\prec$ between the elements of $\cost$ is defined as $a \prec b$ if and only if $a \preceq b$ and $a \neq b$).
\comPC{OK, we are assuming that we have the equality relation for the cost values...}

\problem{The Pareto problem}{Given a TDN $N = \langle G=(V,E),\alpha,\gamma,\thor\rangle$, a cost function $\gamma$ along with its cost combination function $\oplus$ and its cost comparison relation $\preceq$, a source node $s\in V$, and a starting time $t_0\in\thor$, compute all pairs $(t,c)\in\thor\times\cost$ for which there exists a Pareto $t_0$-optimal path $\tpath P\in\allpaths sd$ such that $t=\alpha_{\tpath P}(t_0)$ and $c=\gamma_{\tpath P}(t_0)$.}

As far as we know, this is the first time that this problem is considered in its generality (even if, as we said in the introduction, some specific cases of this problem corresponding to specific cost functions have been already considered in the literature). In the rest of the paper we will first show how the Pareto problem can be solved in the case of point-availability TDNs and of cost functions satisfying some very natural properties, and we will then show several applications of our solution. 



==> oldapplications.tex <==
\section{Applications}
\label{sec:applications}

In this chapter we will show several possible applications of the Algorithm proposed in Section \ref{sec:algorithm}. All the problems listed here will be stated and solved in a $one-to-all$ variation and considering earliest arrival time as the first of the Pareto criteria. However, it is also possible to apply the Algorithm as specified in Section \ref{subsec:ato} and solve the $one-to-all$ variation with respect to latest departure, without any differences on the complexity.


\com{LV: do we formally state Fewest hop path can be solved in time ... and so on ?}

\com{LV: We have to say something about how to compute not only the optimum cost but also a path with this cost.}

\subsection{Fewest hops}\label{minhops}

    
    \com{FB: we need to introduce this problem with a possible application: social networks?}
    
    Consider the problem of finding the minimum number of edges required by a path in a temporal network to reach each possible destination from a given source node. It is possible to apply Algorithm \ref{paroptalg} in order to solve this problem on a temporal network.
    %formalized as the model used in this paper.
    
	Consider the set of costs $W = \mathbb{N}$ and assign to each edge $e = (u,v,\bar{t},l,c)$ the cost $c=1$. The function $\oplus$  is defined as the sum between natural numbers $+ : \mathbb{N} \times \mathbb{N} \longrightarrow \mathbb{N}$. The $\prec$ ordering is defined as the natural ordering $<$ of integers.
	The cost function $C : \mathcal{P} \longrightarrow \mathbb{N}$, induced by the operation $\oplus$, given a temporal path $P = \langle e_1,e_2, \dots, e_k \rangle$, returns the cost $C(P) = k$, namely the number of hops that compose it. Observe that the function $\oplus$ satisfies the istonocity property, thus we are under the hypothesis to apply correctly Algorithm $\ref{paroptalg}$.
	
	Finally, to obtain the minimum number of hops needed by a temporal path to reach a node $v$ from the source $s$, it suffices to look at the cost of the last pair in $PS_v$.
	
	\com{LV: to intro :}
	As for the knowledge of the authors, this is the first algorithm provided to solve this problem with this complexity.
	
	
\subsection{Shortest delay} 

    The classical problem of computing shortest paths in static graphs can be translated in temporal graphs as computing the paths with minimum duration defined as the sum of the delay of the edges. 
    
    In order to solve this kind of problem exploiting Algorithm \ref{paroptalg} we proceed as follows.
    We consider the set of costs $W = \mathbb{R}^+$ and we assign to each edge $e = (u,v,\bar{t},l,c)$ the cost $c=l$. The function $\oplus$  is defined as the sum between real positive numbers $+ : \mathbb{R}^+ \times \mathbb{R}^+ \longrightarrow \mathbb{R}^+$. It  satisfies the isotonicity property for the natural ordering $<$ over reals and induce a cost function $C : \mathcal{P} \longrightarrow \mathbb{R}^+$. This cost function will allow us to find the shortest paths because, given a temporal path $P = \langle e_1,e_2, \dots, e_k \rangle$, its cost is $C(P) = \sum_{i=1}^k l_i$.
	Finally, once the algorithm is executed, in order to obtain the cost of the shortest path from the source $s$ to each node $v \in V$, it suffices to read the cost of the last pair in $PS_v$.
	
	\com{LV: to intro:}
	The most natural comparison against the literature can be made with the algorithm proposed by Wu et. al. \cite{Wu2014Path}. The two algorithms will perform very similar operations, and the computational complexity reached are the same. 
	%\com{FB: The complexities are written slightly different but we can still say that are the same right?
	% The algorithms are basically the same.}
	
\subsection{Profile}\label{latdeptime} 
    
    A classical problem in temporal networks, motivated by transport applications, is to compute, for each possible departure time, the earliest arrival time from a fixed source to a possible destination or even to all destinations. The function giving the earliest arrival time as a function of the departure time is often called a profile.
    
    In our setting, it possible to solve this problem by computing for each node $v$ the Pareto set $PS_v$ containing the values $(arr\_time,dep\_time)$ of a Pareto optimal path with respect to these two criteria where earlier arrival time and latest departure time are preferred. The Pareto set $PS_v$ describes the profile from the source to $v$ in the following way. If we consider two consecutive pairs in $PS_v$, $(arr\_time_1,dep\_time_1)$ and $(arr\_time_2,dep\_time_2)$, they are such that $arr\_time_1 < arr\_time_2$ and $dep\_time_1 < dep\_time_2$ by Pareto optimality; in particular we can deduce that $\forall t \in (dep\_time_1, dep\_time_2]$ the earliest arrival time is $arr\_time_2$ since $PS_v$ contains all Pareto optimal pairs and no pair can have departure time in-between $dep\_time_1$ and $dep\_time_2$. 
    %if by contradiction there exists t \in (dep\_time_1, dep\_time_2] such that there exists a path with arrival time  arr\_time_t <  arr\_time_2, then (arr\_time_t,t) would belong to PS_v, and would be postioned in between (arr\_time_1,dep\_time_1) and (arr\_time_2,dep\_time_2)
    %\com{FB: Do I need to justify this? See commented lines}
    
    In order to solve this problem through the application of Algorithm \ref{paroptalg}, we first define the set of costs as $W = \mathbb{R}$ and assign to each edge $e = (u,v,\bar{t},l,c)$ the cost $c=\bar{t}$. We consider the function $\oplus : \mathbb{R} \times \mathbb{R} \longrightarrow  \mathbb{R} $ defined as $\oplus(a,b) = a$. This guarantees that the induced cost function $C : \mathcal{P} \longrightarrow \mathbb{R}$ works as intended: given a temporal path $P = \langle e_1,e_2, \dots, e_k \rangle$, its cost is $C(P) = \bar{t}_1$, namely the departure time of the first edge and also of the path itself. The $\prec$ ordering is the reverse of the natural ordering: $t_1\prec t_2$ if and only if $t_2 > t_1$. The isotone property comes from the equality $c\oplus c'=c$.
    
	
\subsection{Shortest fastest} 
    The concept of \emph{shortest fastest} paths is introduced by Latapy et. al. \cite{Latapy2018} in a linkstream model to describe the paths with fewest hops among the paths with minimal total duration defined as the difference between arriving and starting times of the path. 
    \com{LV: the following depends on how the link stream is represented (full list of temporal edges vs intervals):}
    Even if it is not possible to reduce the instances of the linkstream model used in their paper to the one we use here, it is possible to adapt this concept to our model using the Multicriteria method. 
    Let us consider the set of costs $W_1 = \mathbb{R}$ and $W_2 = \mathbb{N}$. To each edge $e$ is assigned a cost $c \in W = W_1 \times W_2$, such that the first component is the departure time of the edge and second one is 1. Namely, the edges can be written as $e = (u,v,\bar{t},l,c)$, where $c = (\bar{t},1)$.  The function $\oplus_1 : \mathbb{R} \times \mathbb{R} \longrightarrow  \mathbb{R} $  defined as $\oplus_1(a,b) = a$, will lead, as explained in Section \ref{latdeptime}, to a cost function $C_1 : \mathcal{P} \longrightarrow W_1$ that returns the starting time of the paths with associated ordering $\prec_1=>$. The function $\oplus_2$ defined as the sum between natural numbers $+ : \mathbb{N} \times \mathbb{N} \longrightarrow \mathbb{N}$ will lead, as explained in Section \ref{minhops}, to a cost function $C_2 : \mathcal{P} \longrightarrow W_2$ that return the number of edges that compose the paths with associated ordering $\prec_2=<$. Combining these functions as explained in \ref{multicrit} allows us to compute the values of the Pareto optimal paths with respect to arrival time and a cost that has the departure time in the first component and the number of hops in the second one. Notice that these values do not necessarily correspond to shortest fastest paths, however the values that correspond to the paths we are looking for are included in the values we computed. For each Pareto set it suffices to extract the triplet $(arr\_time, (dep\_time,hops))$ such that $arr\_time-dep\_time$ is minimal among the triplets in the Pareto set. 
    %Since Algorithm \ref{paroptalg} adds at most two pair per iteration, the total number of triplets in the Pareto sets is $O(|E|)$, thus extracting these values will not change the complexity of the algorithm.
    %\com{FB: Do I need to justify more these facts?}
    This final scan is linear and the overall complexity is within a constant factor of that of Algorithm~\ref{paroptalg}.

\com{LV: to intro:}
    We can compare the performance of this algorithm with a result obtained by \cite{simard}. In this paper the author provide an algorithm to compute shortest fastest paths with a linkstream model that is not comparable to ours. However, in order to compare to the literature, Simard also provides an algorithm to compute the values of shortest fastest paths, in a more classical model. In particular this model is equivalent to ours, but additionally requires the restrictive hypothesis that each edge has the same delay, and to work properly, this delay has to be small. The computational complexities of our and Simard algorithm are equal, however ours solves the problem in a more general setting.
    
    



\subsection{Highest reliability}

    In many applications of temporal networks, that range from public transport to epidemic modeling, it can be interesting to model the fact that edges might \emph{fail}, namely the connection will not occur in the actual development of the modeled events. In order to describe this property it is possible to add label, in our setting a cost, to the edges that represents the reliability of the edge, in particular we consider the of the label $c \in [0,1]$ being the probability that the edge does not fail. In this case we want to define the cost of a path $P = \langle e_1, \dots, e_k \rangle$ as the probability that it will be possible to travel across it, namely none of its edges fails. We assume independance of failure events. Thus,  we define the set of cost as $W = [0,1]$, the order $\preceq$ as $\geq$ and the operator $\oplus : [0,1] \times [0,1] \longrightarrow [0,1]$ as the standard product between real numbers. In this way, we obtain the induced cost function $C : \mathcal{P} \longrightarrow [0,1]$ to be the function that assigns to a path $P = \langle e_1, \dots, e_k \rangle$ the quantity $C (P) = \prod_{i=1}^k c_i$, which is the probability that $P$ does not fail.
    Note that $\oplus$ satisfies the isotonicity property as multiplying by a non-negative number preserves order. We can apply Algorithm \ref{paroptalg} to correctly find the set of values of the Pareto optimal paths with respect to earliest arrival time and highest reliability.
    
    Moreover, it is also possible to use this cost in combination with others as previously explained. For example, if we consider as first cost the departure time and the reliability as the secondary cost, it is possible to compute the most reliable path among the shortest path in terms of duration, in a similar fashion to the shortest fastest case.
    
    The independence of edge failures is a simplifying assumption. A more realistic scenario for public transport would be assume line failures: either all edges of a line fail or none.
    %LV: don't see how to justify previous setting
    % This could be modeled in the previous setting by ??

\subsection{Min max} 
    
    A classical graph problem, which study is motivated by several applications, is the min max path problem. The scenario is the following. To each edge is assigned a label, that in our case corresponds to the cost field of the edges, and the smaller the label is, the more the edge is preferable. The cost of a path is the maximum label of the edges that form the path. This means that we are interested in minimizing the maximum label present in the path.
    
    In order to model this problem we can proceed this way. We define the set of cost as $W = \mathbb{N}$, the order $\preceq$ as $\leq$ and the operator $\oplus: \mathbb{N} \times \mathbb{N} \longrightarrow \mathbb{N} $ as the $\max$ function. This way the induced cost function $C : \mathcal{P} \longrightarrow \mathbb{N}$ assigns to each path the maximum label of the edges the path goes through. Since $\oplus$ satisfies the isotonicity property, we are under the hypothesis to apply Algorithm \ref{paroptalg} to obtain the set of values of the Pareto optimal paths with respect to earliest arrival time and minimum max label the paths goes through.
    
    It is also possible, to solve in an analogous way, the max min problem, that is often used to model the problem of finding paths with largest bottleneck in capacitated networks.
    
    
    % Often in transport networks there is the necessity to model the fact there are some \emph{zones} in the network that are more preferable than others, depending for examples on the fares applied or the centrality in the network. A possible way to do this is assigning a label to each edge, in our case a cost $c \in \mathbb{N}$, that identifies the zone the edge belongs to. The smaller the label, the more the zone is preferable. We thus define the set of cost as $W = \mathbb{N}$, the operator $\oplus: \mathbb{N} \times \mathbb{N} \longrightarrow \mathbb{N} $ as the function $\max$. This way the induced cost function $C : \mathcal{P} \longrightarrow \mathbb{N}$ assigns to each path the maximum label of the zones the path goes through. Since $\oplus$ satisfies the isotonicity property, we are under the hypothesis to apply Algorithm \ref{paroptalg} to obtain the set of values of the Pareto optimal paths with respect to arrival time and the zone the paths goes through.
    
    % Again, it is possible to combine this cost with other costs analyzed in this chapter, in order to obtain more specific criteria.
    




==> oldgeneralpaths.tex <==
\section{Solving the Pareto problem in point-availability TDNs}
\label{sec:algorithm}

\textbf{Model:} 
% %Use natural or real timestamps? The algorithm works correctly in both cases. However, if we use real timestamps we cannot obtain a complexity that depends on the maximum length L of edges, because there can be more than L Pareto optimal pair (t,c) such that t \in [\bar{t} - L, \bar{t}]. Even so, I suggest to real time stamp, obtain a complexity that depends on the degree of the edges, and then maybe write an observation that in special case of natural timestamps it is possible to obtain a finer complexity.
We work on a temporal network $G = (V,E)$ where $V$ is the set of nodes and $E$ is the set of temporal connections; we consider also a set of costs $W$, totally ordered by $\preceq$. An edge $e \in E$ is a quintuple $(u,v,\bar{t},l,c)$, where $u$ is the departure node, $v$ is the arrival node, $\bar{t} \in \mathbb{R}$ is the departure time from node $u$, $l \in \mathbb{R}^+_0$ represents the delay due to the travel time, finally $c \in W$ is the cost of the edge. We allow edges with $0$ length under a specific condition: the set of edges that have same departure time and length $l=0$ must not contain any loops, and thus is topologically orderable.
% A temporal path $P$ is a non-empty sequence of edges $\langle e_1,e_2, \dots, e_k \rangle$, where $e_i = (u_i,v_i,\bar{t}_i,l_i,c_i)$, such that $\bar{t}_{i+1} \geq \bar{t}_i + l_i$. In other words, the departure time of each edge of the path has to be greater than the arrival time of the previous one.

\textbf{Problem:} 
% The cost function $C : \mathcal{P} \longrightarrow W$, that assigns to each path a cost, is defined through a function $\oplus : W \times W \longrightarrow W$. 
% Let $P = \langle e_1,e_2, \dots, e_k \rangle$ be a path of length $k$. If $k=1$ we define $C(P) = c_1$, where $c_1$ is the cost of the unique edge of $P$. If $k > 1$ we define recursively the cost of the path as $C(P) = C(\langle e_1,e_2, \dots, e_{k-1} \rangle) \oplus c_k$, where $c_k$ is the cost of the last edge of $P$. 

The problem we are going to solve is the following. We want to compute the set of Pareto optimal values of the paths from a given source to all the possible destinations, with respect to two criteria: arrival time and cost. A path $P$ from $s$ to $d$, with arrival time $t$ and cost $c$, is \emph{Pareto optimal} among the paths from $s$ to $d$, if there is no path $P'$ from $s$ to $d$, with arrival time $t'$ and cost $c'$, such that $t' < t$ and $c' \preceq c$, or $t' \leq t$ and $c' \prec c$. The relation $\prec$ between the elements of $W$ is defined as $a \prec b$ if $a \preceq b$ and $a \neq b$.

As we said in the introduction, we assume that the cost combination function $\oplus$ satisfies the following property.

\begin{property}[Isotonicity]\label{isoprop}
    Let $c_1, c_2 \in W$ such that $c_1 \preceq c_2$, then $c_1 \oplus c \preceq c_2 \oplus c$ for any $c \in W$.
\end{property}
This property guarantees that for any two paths with same source and destination, $P_{su}^1$ and $P_{su}^2$, and costs $c_1 = C(P_{su}^1)$, $c_2 = C(P_{su}^2)$ such that $c_1 \preceq c_2$, and each edge $e$ that can be concatenated to both of them, the cost of $P_{su}^2$ concatenated with $e$ is not better than the cost of $P_{su}^1$ concatenated with $e$. The isotonicity property also allows to state the following lemma.


% \begin{lemma}\label{prefopt}
%     Given a Pareto optimal path $P$ from a node $s$ to a node $d$, there exists a path from node $s$ to $d$ \emph{equivalent} to $P$ (i.e. with same arrival time and same cost) such that each prefix of this path is Pareto optimal. 
% \end{lemma}
% \begin{proof} %is it understandable?
% Let $P$ be a Pareto optimal path, from node $s$ to node $d$. Let $e = (v,d,\bar{t}, l, c)$ be the last edge of $P$, thus $\bar{t} + l$ is the arrival time of $P$. Now let $\tilde{P}$ be a path from $s$ to $v$ that has optimal cost among the paths from $s$ to $d$ that have arrival time less or equal to $\bar{t}$. Consider the path $P' = \langle \tilde{P},e \rangle$. $P'$ has the same arrival time of $P$, because they end the path with the same edge, and it also has the same cost thanks to Property \ref{isoprop}. This way we obtained a path $P'$ with a certain length $k$, \emph{equivalent} to $P$, such that its prefix of length $k-1$ is also Pareto optimal. We can iterate this process on the last but one prefix of the path obtained, which in this case is $\tilde{P}$, until we find path such that all its prefixes are Pareto optimal. 
% Note that during the iteration the path obtained may change in length. At the end of iteration $i$ we obtain a path $P^i$ of length $h$ such that all its prefixes of length greater than $h-i$ are Pareto optimal. After a number of iterations dominated by the maximum length of a Pareto optimal path we conclude.
% \com{LV: A proof by induction (on the number of edges of the path) would be more classical.}
% \end{proof}


\begin{lemma}\label{prefopt}
    %  Given a Pareto optimal path $P$, from a node $s$ to a node $d$, with length greater than 2, there exists a path $P'$ with same source and destination \emph{equivalent} to $P$ (i.e. with same arrival time and same cost), such that also its maximum length prefix is a Pareto optimal path. 
     Given a Pareto optimal path $P=\langle e_1,e_2, \dots,e_k\rangle$, from a node $s$ to a node $d$, with length greater than 2, there exists a path $P' = \langle e_1',e_2',\dots,e_h'\rangle$ with same source and destination \emph{equivalent} to $P$ (i.e. with same arrival time and same cost), such that also its maximum length prefix $\langle e_1',e_2',\dots,e_{h-1}'\rangle $ is a Pareto optimal path. 
\end{lemma}
\begin{proof}
    Let $P= \langle e_1,e_2,\dots,e_k \rangle$ be a Pareto optimal path  from $s$ to $d$, with length $k\geq 2$, and $e_k = (u,d, \bar{t},l,c)$ its last edge. Let us consider a path $\tilde{P}$ from $s$ to $u$ that has optimal cost among the path from $s$ to $u$ that have arrival time less or equal to $\bar{t}$. We define $P'$ as $\langle \tilde{P},e_k\rangle$. $P'$ is a valid temporal path and has the same arrival time of $P$; its cost cannot be less than the cost of $P$ because $P$ is Pareto optimal, it cannot be greater because of Property \ref{isoprop}, thus $P'$ is equivalent to $P$, and its maximum length prefix, which is $\tilde{P}$, is also a Pareto optimal path.
\end{proof}

\com{FB: The statement of the Lemma rewritten in this way is faster to prove and does not change the proof of correctness of the algorithm.}


\textbf{Algorithm:}
We denote with $PS_u$ the Pareto set associated to node $u \in V$ that contains all pairs $(arrival\_time,cost)$ of the Pareto optimal paths from the source to node $u$. The pairs $(t,c)$ in this Pareto sets are ordered by increasing $t$ values.

We assume that the set of temporal edges is ordered by increasing arrival time $\bar{t} + l$, prioritizing edges with length greater than $0$, and  among the edges that have length $0$ and the same arrival time we consider them ordered topologically.

%add case where te new pair dominates the very last element of the Pareto set (they have same arrival time).

\begin{algorithm}[H]
\SetAlgoLined
\SetKwInOut{Input}{input}
\Input{$G = (V,E)$, $s \in V$}

\ForEach{$u \in V$}{
$PS_u \gets \emptyset$\;
}

\ForEach(\tcc*[f]{scanning $E$ as explained above}){$e=(u,v,\bar{t},l,c) \in E$}{
    %$\{(t_1^u,c_1^u), \dots, (t_k^u,c_k^u)\} \gets PS_u$\;
    %$\{(t_1^v,c_1^v), \dots, (t_h^v,c_h^v)\} \gets PS_v$\;
    \If{$u = s$}{
        $\updateps (PS_v,\bar{t} +l,c)$\; \label{alg:case1}
        % \uIf{$PS_v = \emptyset$}{
        %     append $(\bar{t} + l,c)$ to $PS_v$\;
        % }
        % \uElse{
        %   let $(t^v,c^v)$ be the pair with greatest arrival time $t^v$ in $PV_v$\;
        %   \tcc{we have $t^v\le \bar{t}+l$}
        %   \If{$c \prec c^v$}{
        %     \If{$t^v = \bar{t} + l$}{
        %         remove $(t^v,c^v)$ from $PS_v$\;
        %     }
        %     append $(\bar{t} + l,c)$ to $PS_v$\;
        %   }
        % }
    }
    \If{%$PS_u \neq \emptyset$ and $t_1^u \leq\bar{t}$
    $PS_u$ contains a pair $(t,c)$ with $t\leq \bar{t}$
    }{
        %$i \gets \max \{1 \leq j \leq k : t_j^u \leq \bar{t}\}$\;
        let $(t^u, c^u)$ be the pair in $PS_u$ with greatest arrival time $t^u\leq \bar{t}$\;
        %\tcc{LV: TODO: code bellow is similar to before, we should insert a function to factorize code}
        $\updateps (PS_v, \bar{t} + l, c^u \oplus c)$\; \label{alg:case2}
        % \uIf{$PS_v = \emptyset$}{
        %     append $(\bar{t} + l,c^u \oplus c)$ to $PS_v$\;
        % }
        
        % \uElseIf{$c^u \oplus c \prec c_h^v$}{
        %     \If{$t_h^v = \bar{t} + l$}{
        %         remove $(t_h^v,c_h^v)$ from $PS_v$\;
        %     }
        %     append $(\bar{t} + l,c^u \oplus c)$ to $PS_v$\;
        % }
    
    }
    
}
\SetKwFunction{UpdatePS}{\updateps}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\UpdatePS{$PS,t,c$}}{
    let $(t^k,c^k)$ be the last pair in $PS$ if it is non-empty\;
    \uIf{$PS = \emptyset$}{
        append $(t,c)$ to PS\;
    }
    \uElseIf{$c \prec c^k$}{
        \If{$t = t^k$}{
            remove $(t^k,c^k)$ from $PS$\;
        }
        append $(t,c)$ to $PS$\;
    }
}
\caption{Pareto optimal temporal paths}
\label{alg:paretoproblem}
\end{algorithm}

\vspace{2cm}

\textbf{Proof of correctness:}
Let us say that the temporal graph is $G = (V,E)$, and $E_k$ is the set of the edges scanned until the $k$-th iteration. We will prove by induction that the Pareto sets at iteration $k$ represent the right Pareto optimal values in the temporal graph $G_k(V,E_k)$. 
%If this is true, than the algorithm returns the correct output.
The correctness of the algorithm follows from that property for $k=|E|$.

%We can reason by induction. Base case is 
%LV you cannot write : okay
The property is satisfied for $k=0$: the Pareto sets are all empty because there are not paths with positive length when $E_0 = \emptyset$. 
%LV: You cannot write : Let's see 
%what happens in the induction step. 
Now suppose that the property holds for $k$ and let us prove it for $k+1$. Denote with $e = (u,v,\bar{t},l,c)$ the edge selected at iteration $k+1$. The temporal paths in $G_{k+1}$ that were not present in $G_k$, and that  possibly lead to an update of the Pareto sets, are the paths that go through edge $e$.
Let us distinguish two cases: 
\begin{itemize}
    \item $l>0$: since the edges are ordered by increasing arrival time, there cannot be edges in $G_{k+1}$ that depart from $v$ at time $\bar{t} + l$ or later. This because, if an edge departs at time $\bar{t} + l$ or later it has greater arrival time than $e$, except in the case it has length 0 and departs at time $\bar{t} + l$, but due to the order we defined also this case is not possible (among the edges with same arrival time the ones with length gretaer than $0$ have priority).
    Thus the new temporal paths, generated by adding $e$ to the network $G_k$, have $e$  as their last edge.
    \item $l=0$: also in this case there cannot be any edges that depart from $v$ after time $\bar{t} + l$. However, $E_{k+1}$ can contain edges that have $\bar{t} + l$ as departure time and have length $0$. Since we are scanning the edges with length $0$ by their topological order, none of these edges depart from $v$. Thus, again, the new paths that contain edge $e$ have $e$ as their last edge.
\end{itemize}

This means that the only Pareto set that might be updated during this iteration is the Pareto set of $v$. 

First of all we have to distnguish the case where the edge considered is starting a new path, namely the case where the departure node of the edge is also the source. The edge constitutes a Pareto optimal path itself if  $(\bar{t} + l,c)$ is not dominated by the last element of $PS_v$. It is sufficient to check the last element of $PS_v$ because it is the one with better cost and $\bar{t} + l$ is greater or equal to every arrival time in $PS_v$.

Now consider the case in which $e$ extends a previous Pareto optimal path. Note that all the values corresponding to the Pareto optimal paths with destination $u$, that can be concatenated with $e$, are already included in the Pareto set of $u$. Thus, thanks to Lemma \ref{prefopt}, in order to update the Pareto set of $v$ with the new values, corresponding to the Pareto paths with destination $v$ that have $e$ as their last edge, we just need to examine the Pareto set of $u$. Moreover, %thanks to Property \ref{isoprop}, 
we are just interested in the Pareto optimal paths, that arrives in $u$, no later than $\bar{t}$, so that cancatenating $e$ produces a valid path. Among those paths, we only have to consider the one with lowest cost as concatenating $e$ will always produce a path arriving at the same time $\bar{t} + l$. Note that this path is also the one having greatest arrival time among those arriving no later than $\bar{t}$ as we consider only Pareto optimal paths.
%This is because each Pareto optimal path with destination $u$ and arrival time no greater than $\bar{t}$, 
%When concatenated with $e$, will have the same arrival time $\bar{t} + l$. Thus we are interested in the path from $s$ to $u$, that, once concatenated with $e$, will have a better cost.
Thanks to Property \ref{isoprop} we know that this path produces the one with better cost after concatenation with edge $e$. %ong the paths that arrive in $u$ before $\bar{t}$. 
%In particular, the one with better cost is the one with greatest arrival time, otherwise it would be dominated.
Using the function $\oplus$ we find the cost of the path extended with edge $e$, and once again it is enough to check if it is dominated by the last element of $PS_v$.

Note that when we add a new pair $(arrival\_time,cost)$ to a Pareto set, this pair cannot dominate any pair already present except for the last one, because it might have the same arrival time (all the other pairs have earlier arrival time, thus cannot be dominated). If this is the case we need to remove it from the Pareto set.





% \com{LV: The next paragraph is more a rephrasing of the algorithm than a proof.}

% Now that we restricted the set of paths that might update the Pareto set of $v$ to at most one possible candidate, we need to correctly compute its values of arrival time and cost, and then perform the update. 
% First of all we distnguish the case where the edge considered is starting a new path, namely the case where the departure node of the edge is also the source. In this case, in order to understand if the edge considered constitutes a Pareto optimal path, we just need to check if $(\bar{t} + l,c)$ is dominated by any pair in $PS_v$; if it is not the case, we add it.
% \com{LV: Need to justify here that it is sufficient to check that the last pair does not dominate it.}

% \com{LV: Again the next paragraph is a rephrasing of the algorithm, we do not really need it.}
% Then, we need to compute the cost of the only possible candidate path the we identified above, if its values are not dominated we add them to the Pareto set of $v$. To do this, we identify the pair $(arrival\_time,cost)$ in $PS_u$ that has the latest arrival time, while preserving the possibility of adding $e$ to the path (i.e. with time less than $\bar{t}$). If this pair does not exist, we do not do anything, because there are no paths from $s$ to $u$ that can be extended with $e$. Once this pair of $PS_u$ is identified we compute the cost of the cadidate path trough the function $\oplus$. If the values obtained are not dominated by other pairs in $PS_v$ we add the new pair to it.

% Note that when we add a new pair $(arrival\_time,cost)$ to a Pareto set, this pair cannot dominate any pair already present except for the last one, because it might have the same arrival time (all the other pairs have earlier arrival time, thus cannot be dominated). If this is the case we need to remove it from the Pareto set.




\textbf{Complexity:}
Suppose that the temporal edges are already ordered as described above. Suppose also that the operation $\oplus$ and the comparison $\prec$ require constant time. The algorithm performs one iteration for each edge scanned. The removal operations that are executed require only to possibly remove the last element of a list, thus these operations require constant time. 

The only operation that does not require constant time is  finding in $PS_u$ the pair  with greatest arrival time $t^u\leq \bar{t}$. We will now give a bound on this operation. Consider for each edge $e=(u,v,\bar{t},l,c)$ the quantity $K_e$, defined as the number of Pareto optimal values $(t,c)$ in $PS_u$ such that $t \in (\bar{t}, \bar{t} +l ]$, and let $K = \max_{e \in E} K_e$. Observe that the pair $(t^u,c^u)$ we are looking for is located exactly before the last $K_e$ elements of $PS_u$. It is possible to proceed in the following way. Let $p$ be the length of $PS_u$, we look at the pairs in position $p$, $p-1$, $p-2$, $p-4$, $p-8$, \dots, until we find, in a certain position $p-k$ (after $O(\log k)$ steps), a pair with time less or equal to $\bar{t}$. Observe that the pair we are looking for is in position between $p-k$ and $p-k/2$; using a binary search we find it in $O(\log k)$ iterations. Since $k \leq 2 K_E$ the total cost to perform this operations is $O(\log K)$. We can conclude that the  on the computational cost of the algorithm is $O(|E| \cdot \log K)$.


% The only operation that does not require constant time is the computation of $\max \{1 \leq j \leq k : t_j^u \leq \bar{t}\}$. Using a binary search the cost of this operation is bounded by the logarithm of the maximum possible length of a Pareto set. Since it is possible to add a new pair to the Pareto set of a node only when is scanned an edge that has this node as arrival node, the maximum length of the Pareto sets is bounded by $\Delta$, the maximum in-degree in the temporal network. This guarantees a bound on the computational cost of $O(|E| \cdot \log(\Delta))$.

%add special case where timestamps and delays are natural numbers.

\textbf{Space Complexity:}
During each iteration the algorithm adds at most two pairs to a Pareto set if the departure node is the source, and at most one pair in the other cases. This guarantees that the total number of pairs in the Pareto sets is bounded by $2 \cdot |E|$, thus the algorithm has linear space complexity.

\begin{subsection}{Multicriteria:}\label{multicrit}
    Let us consider $h$ sets of costs $W_1, \dots, W_h$, totally ordered by a respective relation $\preceq_1,\dots, \preceq_h$, and suppose that to each edge, instead of just one cost, is assigned a total of $h$ costs, one for each set. 
    
    Let us consider, for each $1 \leq i \leq h$, a cost function $C_i : \mathcal{P} \longrightarrow W_i$ that evaluates the cost of the paths in the temporal graph with respect to the $i$-th cost assigned to the edges. We define this function recursively as we did before, through a function $\oplus_i : W_i \times W_i \longrightarrow W_i$ that satisfy the isotonicity property. 
    Let us denote with $W = W_1 \times \dots \times W_h$ and consider  a total lexicographical order $\preceq$ on this set as follows. Let $c_1=(c_1^1, \dots,c_1^h), c_2=(c_2^1,\dots,c_2^h)$ be two elements of $W$:
    
    \begin{equation}
        c_1 \preceq c_2 \Longleftrightarrow c_1 = c_2 \text{ or } c_1^i \prec_i c_2^i \text{ for the first index $i$ such that $c_1^i \neq c_2^i$},
    \end{equation}
    
    where $\prec_i$ is the strict order on $W_i$ induced by $\preceq_i$. It is now possible to define an operation $\oplus : W \times W \longrightarrow W$ that satisfy the isotone property with respect to $\preceq$:
    
    \begin{equation}
        c_1 \oplus c_2 = (c_1^1, \dots,c_1^h) \oplus (c_2^1,\dots,c_2^h) \coloneqq (c_1^1 \oplus_1 c_2^1, c^2_1 \oplus_2 c^2_2, \dots, c_1^h \oplus_h c_2^h).
    \end{equation}
    
    Finally, we can define recursively a cost function $C : \mathcal{P} \longrightarrow W$ relying on $\oplus$. Let $P = \langle e_1, \dots, e_k\rangle$ be a path of length $k$; if $k=1$ we define $C(P)=(c_1^1,\dots, c_h^1)$, where $(c_1^1,\dots, c_h^1)$ are the cost of only edge $e_1$ that belongs to the path; if $k > 1$ we define the cost of the path as $C(P) = C(\langle e_1, \dots, e_{k-1}\rangle \oplus (c_k^1, \dots,c_k^h)$, where $(c_k^1, \dots,c_k^h)$ are the costs of the last edge of the path $e_k$.
    To summarize, we assigned to each edge a cost $c \in W$, defined a cost function $C : \mathcal{P} \longrightarrow W$ through the operation $\oplus$ that satisfies the isotonicity property. Thus, we are working in a model that allows to use Algorithm \ref{paroptalg} correctly. In this way we managed to combine a plurality of costs and prioritize paths with respect do different criteria, provided that an order of importance between them is given.
    Note that this approach is  different from looking for the Pareto optimal values with respect to $h$ different costs of equal importance.
    
\end{subsection}


\subsection{Temporal edges with zero delay}

We now show how zero delays can be tolerated under the following condition on the graphs formed by zero-delay edges at a given time. Given a temporal graph $G$, we define $G_t^0$ as the graph with edges $(u,v,c)$ such that there exists a temporal edge $(u,v,t,0,c)$ in $G$. We say that a graph with cost on edges is \emph{cost transitively closed} when for each pair of edges $(u,v,c)$ and $(v,w,c')$ there always exists an edge $(u,w,c'')$ with $c''\preceq c\oplus c'$. If $\oplus$ is not associative, we additionally require that $d\oplus c''\preceq (d\oplus c)\oplus c'$ for any cost $d$.
\com{LV: is it necessary to consider case $\oplus$ not associative?}
Finally a temporal graph $G$ is said to be \emph{zero transitively closed} when any strongly connected component of  $G_t^0$ is cost transitively closed for all $t$. 

Algorithm~\ref{paroptalg} can then be adapted to take as input any zero transitively closed graph by refining the order in which the temporal edges in $E$ are scanned: we additionally require that the edges with same arrival time $t$ and having delay zero, i.e. those that correspond to edges in $G_t^0$ are given according to a topological order of the strongly connected components of $G_t^0$.

The correctness follows from two facts. First, the cost transitively closed hypothesis allows to consider only paths with at most one edge in any strongly connected component of any $G_t^0$ as any path is dominated by such a path.
Second, the topological ordering assumption ensures that any sequence of edges with zero delay and same arrival time $t$ in a such path are visited in the same order as in the path.

\com{LV: the zero transitively closed property is not necessary when the cost of zero-delay edges is 0...}






\subsection{Path extraction:}

The Algorithm described in \ref{sec:algorithm} computes the values of arrival time and cost of the Pareto optimal paths. In this section we describe how to compute a path that correspond to each value.

In order to do this, we proceed as follows. To each value $(t,c)$ in a Pareto set $PS_v$ we will add two pointers during the execution of the algorithm. Consider the iteration of the Algorithm during which $(t,c)$ is appended to $PS_v$. We add to $(t,c)$ a first pointer to the edge $e = (u,v,\bar{t}_e, l_e,c_e)$ that corresponds to the current iteration. Then, for the second pointer, if $(t,c)$ is added to $PS_v$ through the function $\updateps$ called in line \ref{alg:case2}, we add a pointer to $(t^u,c^u)$ in $PS_u$, otherwise if $(t,c)$ is added to $PS_v$ through $\updateps$ called in line \ref{alg:case1} we add a pointer to $\texttt{null}$, because $e$ is the starting edge of the path.

To extract a path corresponding to a certain values $(t,c)$ in a Pareto set $PS_v$ we will reconstruct the path backwards, from its last edge to the first one. First of all we consider the path $P = \langle e \rangle$, where $e$ is the edge obtained by the first pointer of $(t,c)$. Then we consider the value obtained by the second pointer of $(t,c)$: if it is $\texttt{null}$ we return $P$, if it is a pair $(t^u,c^u)$ we pre-append to $P$ the edge linked by the first pointer of $(t^u,c^u)$ and we iterate this process on its second pointer. 









\begin{subsection}{All-to-one latest departure time problem}\label{subsec:ato}
    
    Consider the same model of temporal network as before, but with a different definition of the cost function $C : \mathcal{P} \longrightarrow W$. This time it is defined recursively backwards with respect to the path, namely, given a path of length $k$, $P = \langle e_1,e_2, \dots, e_k \rangle$, if  $k=1$ we define $C(P) = c_1$, if $k > 1$ we define $C(P) = c_1 \oplus C(\langle e_2,e_3, \dots, e_{k} \rangle)$
    
    Let us now consider the problem of computing the set of Pareto optimal values of the paths from all the possible nodes towards a given destination node, with respect to two criteria: departure time and cost. A path $P$ from $s$ to $d$, with departure time $t$ and cost $c$, is \emph{Pareto optimal} among the paths from $s$ to $d$, if there is no path $P'$ from $s$ to $d$, with departure time $t'$ and cost $c'$, such that $t' > t$ and $c' \preceq c$, or $t' \geq t$ and $c' \prec c$.
    
    Moreover, instead of Property \ref{isoprop} we require the following to hold:
    \begin{property}
          Let $c_1, c_2 \in W$ such that $c_1 \preceq c_2$, then $c \oplus c_1 \preceq c \oplus c_2$ for any $c \in W$.
    \end{property}
    
    This because we will build the paths backwards from the destination to all the possible sources.
    \com{FB: There is also the corresponding of Lemma 1 that could be stated.}
    
    It possible to solve this problem with a slight modification of Algorithm \ref{paroptalg}. We denote with $PS_u$ the Pareto set associated to node $u \in V$ that contains all pairs $(departure\_time,cost)$ of the Pareto optimal paths from node $u$ to the destination node $d$. As before, the pairs $(t,c)$ in this Pareto sets are ordered by increasing $t$ values.

    Consider the set of edges $E$ ordered by decreasing departure time $\bar{t}$, prioritizing edges with length greater than $0$, and  among the edges that have length $0$ and the same arrival time we consider them ordered inversely with respect to the topological order. The Algorithm will scan each edge in $E$ following this order. For each edge $e=(u,v,\bar{t},l,c)$ will verify if the path starting from $u$ to the destination $d$, obtained by concatenating $e$ with the optimal pair extracted from $PS_v$ (namely the one with earlier departure time $t^v\geq \bar{t} + l$), is a Pareto optimal value.
    
    % \begin{algorithm}[H]
    %     \SetAlgoLined
    %     \SetKwInOut{Input}{input}
    %     \Input{$G = (V,E)$, $d \in V$}
        
    %     \ForEach{$u \in V$}{
    %     $PS_u \gets \emptyset$\;
    %     }
        
    %     \ForEach(\tcc*[f]{scanning $E$ as explained above}){$e=(u,v,\bar{t},l,c) \in E$}{
    %         \If{$v = d$}{
    %             $\updateps (PS_u,\bar{t},c)$\;
    %         }
    %         \If{$PS_u$ contains a pair $(t,c)$ with $t\leq \bar{t}$}{
    %             let $(t^v, c^v)$ be the pair in $PS_v$ with earlier departure time $t^v\geq \bar{t} + l$\;
    %             $\updateps (PS_u, \bar{t}, c \oplus c^v)$\;
    %         }
    %     }
    %     \SetKwFunction{UpdatePS}{\updateps}
    %     \SetKwProg{Fn}{Function}{:}{}
    %     \Fn{\UpdatePS{$PS,t,c$}}{
    %         let $(t^1,c^1)$ be the first pair in $PS$ if it is non-empty\;
    %         \uIf{$PS = \emptyset$}{
    %             append $(t,c)$ to PS\;
    %         }
    %         \uElseIf{$c \prec c^1$}{
    %             \If{$t = t^k$}{
    %                 remove $(t^1,c^1)$ from $PS$\;
    %             }
    %             append $(t,c)$ to $PS$\;
    %         }
    %     }
        
    %     \caption{All - to - one Pareto optimal temporal paths }
    %     \label{ato_paroptalg}
    % \end{algorithm}
    
    \com{FB: The proof is very similar to the one of the previous Algorithm.}
    
\end{subsection}

==> shortestpaths.tex <==
\section{General paths}

\textbf{Model:} edge $(u,v,\bar{t},l)$ departs from $u$ at $\bar{t}$ and arrives in $v$ at $\bar{t}+l$, edge $(v,w,\bar{t}',l')$ can follow $(u,v,\bar{t},l)$ in a temporal path when $\bar{t}'>=\bar{t}+l$, $t$ and $l$ are not necessarily integers.

For each node $v \in V$, I want to create a profile $f_v(t)$ which for each time $t$ returns the minimum number of hops to reach $v$ from $s$ arriving no later than time $t$. It will be a piecewise constant function.

\textbf{Input:} node $s$, array $E$ of temporal edges $(u,v,\bar{t},l)$

\textbf{Output:} for each $v$, the length of a shortest temporal path from $s$ to $v$ (in number of hops)

\textbf{Algorithm:}

\begin{itemize}
    \item We initialize $f_s(t) = 0 \, \forall t$ and $f_v(t) = + \infty \, \forall t \, \forall v \in V \setminus \{s\}$. 
    \item Scan edges $(u,v,\bar{t},l)$ by increasing arrival $\bar{t} +l$:
    \begin{itemize}
        \item Update $f_v(t)$: 
        \begin{equation*}
            f_v(t) =
                    \begin{cases}
                      f_v(t) & \text{if $0 \leq t < \bar{t} + l$}\\
                      min \{f_v(t), f_u(\bar{t}) +1 \} & \text{if $t \geq \bar{t} + l$}
                    \end{cases}    
        \end{equation*}
    \end{itemize}
    \item Return $f_v(t_{\text{max}})$, where $t_{\text{max}}$ = max $\{\bar{t} +l : (u,v,\bar{t},l) \in E\}$.
\end{itemize}

\textbf{Some observations:} Let's say that the temporal graph is $G = (V,E)$, and $E_k$ is the set of the edges scanned till the $k$-th iteration. I would like that the profile functions at iteration $k$ represent the right quantity (the minimum number of hops to reach $v$ from $s$ arriving no later than time $t$) in the temporal graph $G_k(V,E_k)$. If this is true than the algorithm return the correct output.
We can reason by induction. Base case is okay. Let's see what happens in the induction step. Suppose that the property holds for $k$ and prove it for $k+1$. Denote with $e = (u,v,\bar{t},l)$ the edge selected for iteration $k+1$. The information that $e$ is adding to the network, is that it is possible to reach $v$ at time $\bar{t} + l$ with $f_u(\bar{t}) +1 $ hops. The update of the profile $f_v(t)$ capture this new information. However, if there are other nodes whose minimum temporal hop paths go through $v$ after time $\bar{t} + l$, their profile can be now incorrect (in particular now might be shorter). This is the reason why the scanning order of the edges matter. In fact, there cannot be such kind of shortest paths if $\nexists e = (v,w,\bar{t}',l') \in E_k$ such that $\bar{t}' \geq \bar{t}+ l$.
\begin{itemize}
    \item if we order the edges by increasing departure time: each edge $(v_1,v_2,\bar{t}',l') \in E_k$ is such that $\bar{t}' \leq \bar{t} < \bar{t} +l$. So this is a correct order to scan the edges.
    \item if we order the edges by increasing arrival time:  each edge $(v_1,v_2,\bar{t}',l') \in E_k$ is such that $\bar{t}'< \bar{t}' +l' \leq \bar{t} + l$. So this is also a correct order to scan the edges.
\end{itemize}

In particular I think that the second one is a preferable order because, if the edges are order by arrival time, when we have to compute $min \{f_v(t), f_u(\bar{t}) +1 \}$ for each $t \geq \bar{t} + l$, it will be necessary just one comparison since $f_v(t)$ is constant for $t \geq \bar{t} + l$. This is true because the breakpoints  in these piecewise constant functions are present only at time instants which are the arrival times of some edge already scanned.

Note that, at each iteration after scanning $(u,v,\bar{t},l)$, it is possible to keep stored just the interval $[\bar{t} + l - L, \bar{t} + l]$ for each profile function, since the interval $[0, \bar{t} + l - L)$ will not be needed anymore, and the value of the function after $\bar{t} + l$ is know, because it is constant.

\textbf{Complexity analysis:} We can store the profile functions $f_v(t)$ as $(t_1^v,h_1^v,t_2^v,h_2^v,\dots,t_k^v,h_h^v)$, where $t_i^v$ is the $i$-th breakpoint of $f_v(t)$ and $h_i^v$ is the value at that breakpoint. Suppose also that the length of the profile function is accessible in constant time.
Suppose we are dealing with the $i$-th iteration of the algorithm and the edge scanned is $e = (u,v,\bar{t},l)$. 

Obs: At this point the last breakpoint in each profile function is not greater than $\bar{t} + l$.

The following are the operations we need to compute during this iteration:
\begin{itemize}
    \item Compute $f_v(\bar{t}+l)$: this is easy, we just need to return value at the last breakpoint of $f_v(t)$, namely $h_k^v$. The cost of this operation is $O(1)$.
    \item Compute $f_u(\bar{t})$: the cost of this operation depends if we are working with natural or real labels. Suppose that are natural. We scan the breakpoint of $f_u(t)$ starting from the last one and going backwards. Since the last one is no later than $\bar{t} +l$, in maximum $l$ steps we reach the breakpoint that precedes $\bar{t}$ and then we can return $f_u(\bar{t})$. The cost of this operation is $O(L)$.
    
    I think that is possible to do this with cost $O(\log L)$ if we search the breakpoint desired between that last $L$ breakpoints of the function with binary search, instead of scanning all the breakpoints backwards until we find it.
    \item Compute min$\{f_v(\bar{t}+l),f_u(\bar{t})+1\}$: The cost of this operation is $O(1)$.
    \item Update $f_v(t)$: If the argmin of the previous operation is $f_u(\bar{t}) + 1$ then $f_v(t)$ needs to be updated. In particular, if the last breakpoint of $f_v(t)$ is different from $\bar{t} + l$, the breakpoint needs to be added, otherwise it needs to be replaced. The cost of this operation is $O(1)$. 
\end{itemize}

Thus, if we are working with natural labels, the cost of each iterations is $O(L)$ (or $O(\log L)$ if we can use binary search). Since the number of iterations is $m$ the total cost of the algorithm is $O(m \cdot L)$ (or $O(m \cdot \log L)$.

\textbf{Idea to solve case of length=0: } 

